FairTune: A Bias-Aware Fine-Tuning Framework Towards Fair Heart Rate Prediction from PPG

Foundation models pretrained on physiological data such as photoplethysmography (PPG) signals are increasingly used to improve heart rate (HR) prediction across diverse settings. Fine-tuning these models for local deployment is often seen as a practical and scalable strategy. However, its impact on demographic fairness particularly under domain shifts remains underexplored. We fine-tune PPG-GPT a transformer-based foundation model pretrained on intensive care unit (ICU) data across three heterogeneous datasets (ICU, wearable, smartphone) and systematically evaluate the effects on HR prediction accuracy and gender fairness. While fine-tuning substantially reduces mean absolute error (up to 80%), it can simultaneously widen fairness gaps, especially in larger models and under significant distributional characteristics shifts. To address this, we introduce FairTune, a bias-aware fine-tuning framework in which we benchmark three mitigation strategies: class weighting based on inverse group frequency (IF), Group Distributionally Robust Optimization (GroupDRO), and adversarial debiasing (ADV). We find that IF and GroupDRO significantly reduce fairness gaps without compromising accuracy, with effectiveness varying by deployment domain. Representation analyses further reveal that mitigation techniques reshape internal embeddings to reduce demographic clustering. Our findings highlight that fairness does not emerge as a natural byproduct of fine-tuning and that explicit mitigation is essential for equitable deployment of physiological foundation models.

==> Tables/table2_previous.tex <==
\begin{table*}[!t]
\floatconts
  {tab:Bias_Mitigation_Performance}%
  {\caption{Cross-Dataset Heart Rate Prediction Performance with Bias Mitigation Strategies for 19M PPG-GPT Model.}}%
  {%
    \small
    \begin{threeparttable}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ll|l|c|cc|c}
    \toprule
    \multirow{2}{*}{\textbf{Trainset}} & \multirow{2}{*}{\textbf{Testset}} & \multirow{2}{*}{\textbf{Method}} 
    & \multicolumn{3}{c|}{\textbf{Predictive Performance (MAE ↓)}} 
    & \textbf{Fairness Gap} \\
     & & & \textbf{Total} & \textbf{Male} & \textbf{Female} & \textbf{$|$Male$-$Female$|$} \\
    \midrule
    \multirow{4}{*}{DaLiA} & \multirow{4}{*}{DaLiA} & Unbalanced 
    & 4.28 [4.18--4.36] & 4.55 [4.47--4.70] & 4.06 [3.94--4.17] & 0.49 [0.41--0.63] \\
    \cmidrule{3-7}
    & & IF 
    & \textbf{4.28 [4.15--4.38]} & 4.45 [4.28--4.61] & 4.15 [4.02--4.25] & \textbf{0.30 [0.21--0.45]} \\
    & & GroupDRO 
    & 5.97 [5.79--6.19] & 6.20 [5.89--6.49] & 5.78 [5.58--5.94] & 0.42 [0.15--0.76] \\
    & & ADV 
    & 5.33 [5.12--5.73] & 5.80 [5.62--6.27] & 4.93 [4.70--5.28] & 0.87 [0.75--0.99] \\
    \midrule
    \multirow{4}{*}{DaLiA} & \multirow{4}{*}{BUT-PPG} & Unbalanced 
    & 19.23 [12.61--25.85] & 20.64 [13.84--27.44] & 17.90 [11.52--24.28] & 2.36 [--0.23--4.95] \\
    \cmidrule{3-7}
    & & IF 
    & \textbf{13.44 [11.52--15.36]} & 14.10 [12.86--15.34] & 12.80 [10.21--15.39] & 1.30 [--0.14--2.74] \\
    & & GroupDRO 
    & 15.47 [13.79--17.16] & 15.81 [13.83--17.79] & 15.15 [13.79--16.51] & \textbf{0.68 [--0.10--1.46]} \\
    & & ADV 
    & 14.49 [11.21--17.79] & 14.85 [11.28--18.42] & 14.17 [10.11--18.22] & 0.70 [--0.29--1.65] \\
    \midrule
    \multirow{4}{*}{DaLiA} & \multirow{4}{*}{MIMIC} & Unbalanced 
    & 24.74 [21.71--27.77] & 24.32 [21.57--27.07] & 24.99 [21.83--28.15] & 0.80 [0.42--1.19] \\
    \cmidrule{3-7}
    & & IF 
    & 22.72 [21.54--23.91] & 22.07 [20.78--23.36] & 23.13 [22.00--24.26] & 1.06 [0.91--1.21] \\
    & & GroupDRO 
    & 22.46 [21.05--23.86] & 21.71 [20.20--23.22] & 22.91 [21.62--24.20] & 1.20 [0.90--1.50] \\
    & & ADV 
    & 22.70 [20.05--25.35] & 21.98 [19.06--24.89] & 23.13 [20.63--25.64] & 1.16 [0.71--1.60] \\
    \midrule
    \multirow{4}{*}{BUT-PPG} & \multirow{4}{*}{BUT-PPG} & Unbalanced 
    & 9.94 [9.77--10.14] & 11.54 [11.11--11.73] & 8.40 [7.91--8.87] & 3.15 [2.24--3.81] \\
    \cmidrule{3-7}
    & & IF 
    & 9.94 [9.80--10.12] & 11.54 [11.09--11.74] & 8.40 [7.93--8.85] & 3.13 [2.26--3.81] \\
    & & GroupDRO 
    & 10.87 [10.65--10.96] & 10.96 [10.57--11.31] & 10.79 [10.21--11.33] & \textbf{0.18 [--0.77--0.90]} \\
    & & ADV 
    & \textbf{10.03 [9.90--10.22]} & 11.59 [11.06--12.01] & 8.54 [8.15--8.94] & 3.05 [2.26--3.86] \\
    \midrule
    \multirow{4}{*}{BUT-PPG} & \multirow{4}{*}{DaLiA} & Unbalanced 
    & 17.62 [17.46--17.78] & 21.41 [21.30--21.52] & 14.42 [14.23--14.61] & 6.99 [6.86--7.12] \\
    \cmidrule{3-7}
    & & IF 
    & \textbf{17.65 [17.38--17.92]} & 21.37 [21.10--21.64] & 14.51 [14.25--14.77] & \textbf{6.86 [6.81--6.91]} \\
    & & GroupDRO 
    & 18.18 [17.83--18.53] & 22.04 [21.66--22.42] & 14.92 [14.66--15.18] & 7.12 [7.01--7.24] \\
    & & ADV 
    & 19.47 [18.62--20.31] & 23.35 [22.44--24.25] & 16.19 [15.39--16.99] & 7.15 [6.87--7.44] \\
    \midrule
    \multirow{4}{*}{BUT-PPG} & \multirow{4}{*}{MIMIC} & Unbalanced 
    & 24.74 [24.52--24.95] & 24.21 [23.85--24.57] & 25.06 [24.73--25.39] & 0.85 [0.82--0.88] \\
    \cmidrule{3-7}
    & & IF 
    & 24.62 [24.37--24.88] & 24.09 [23.81--24.37] & 24.95 [24.71--25.19] & 0.86 [0.82--0.89] \\
    & & GroupDRO 
    & \textbf{20.14 [20.01--20.28]} & 18.96 [18.74--19.18] & 20.86 [20.78--20.94] & 1.90 [1.74--2.06] \\
    & & ADV 
    & 24.92 [24.10--25.74] & 24.36 [23.51--25.22] & 25.26 [24.50--26.01] & \textbf{0.89 [0.79--1.00]} \\
    \midrule
    \multirow{4}{*}{MIMIC} & \multirow{4}{*}{MIMIC} & Unbalanced 
    & 9.76 [9.46--10.00] & 11.40 [11.24--11.74] & 8.77 [8.08--9.22] & 2.62 [2.08--3.65] \\
    \cmidrule{3-7}
    & & IF 
    & 9.76 [9.38--10.28] & 11.43 [10.98--12.15] & 8.75 [8.18--9.61] & 2.68 [1.77--3.88] \\
    & & GroupDRO 
    & 11.37 [10.24--12.31] & 12.19 [11.59--12.41] & 10.87 [9.42--12.31] & \textbf{1.32 [0.01--2.48]} \\
    & & ADV 
    & \textbf{10.16 [10.01--10.27]} & 11.69 [11.10--12.58] & 9.23 [8.70--9.77] & 2.46 [1.33--3.88] \\
    \midrule
    \multirow{4}{*}{MIMIC} & \multirow{4}{*}{BUT-PPG} & Unbalanced 
    & 18.68 [16.44--20.93] & 16.17 [14.50--17.84] & 21.10 [18.32--23.88] & 4.93 [3.45--6.41] \\
    \cmidrule{3-7}
    & & IF 
    & 29.64 [26.39--32.89] & 27.72 [24.10--31.34] & 31.48 [28.42--34.54] & 3.76 [2.73--4.80] \\
    & & GroupDRO 
    & 37.02 [29.09--44.95] & 36.14 [26.82--45.46] & 37.86 [30.81--44.91] & \textbf{2.03 [0.54--3.52]} \\
    & & ADV 
    & \textbf{27.21 [20.34--34.08]} & 24.73 [17.18--32.29] & 29.58 [23.45--35.72] & 4.85 [3.38--6.32] \\
    \midrule
    \multirow{4}{*}{MIMIC} & \multirow{4}{*}{DaLiA} & Unbalanced 
    & 34.95 [31.33--38.57] & 38.61 [35.20--42.02] & 31.86 [28.00--35.72] & 6.75 [6.19--7.31] \\
    \cmidrule{3-7}
    & & IF 
    & \textbf{25.24 [22.26--28.23]} & 29.36 [26.54--32.18] & 21.77 [18.67--24.87] & 7.59 [7.24--7.94] \\
    & & GroupDRO 
    & 42.15 [39.30--44.99] & 46.12 [43.65--48.59] & 38.79 [35.62--41.96] & 7.33 [6.64--8.02] \\
    & & ADV 
    & 36.54 [34.12--38.95] & 40.88 [38.50--43.27] & 32.87 [30.49--35.25] & \textbf{8.01 [7.38--8.64]} \\
    \bottomrule
    \end{tabular}
    }
    \begin{minipage}{\linewidth}
    \scriptsize
    Values are reported as median [95\% confidence interval] unless otherwise indicated. IF = Instance-weighted Fairness (Balanced training approach). Best performance values are shown in \textbf{bold} for each dataset pair.
    \end{minipage}
    \end{threeparttable}
  }
\end{table*}

==> Tables/table4.tex <==
\vspace{-3.0ex}
\begin{table*}[h]
\centering
\small
\caption{Mean absolute error (MAE) and fairness gap in heart rate prediction across training-testing dataset combinations and bias mitigation methods. MAE values are shown separately for total population and subgroups. Fairness gap is defined as the absolute difference between male and female MAEs (|Male – Female|). All values are reported with 95\% confidence intervals.}
\begin{tabular}{llc|ccc|ccc}
\toprule
\multirow{2}{*}{Trainset} & \multirow{2}{*}{Testset} & \multirow{2}{*}{Metric} 
& \multicolumn{3}{c|}{Mean Absolute Error (MAE)} 
& \multicolumn{3}{c}{Fairness Gap (|M–F|)} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & & IF & GroupDRO & ADV & IF & GroupDRO & ADV \\
\midrule

\multirow{4}{*}{Dalia} & \multirow{4}{*}{BUT-PPG} 
& Total  & 13.44 [11.52–15.36] & 15.47 [13.79–17.16] & 14.49 [11.21–17.79]
& – & – & – \\
& & Male   & 14.10 [12.86–15.34] & 15.81 [13.83–17.79] & 14.85 [11.28–18.42]
& – & – & – \\
& & Female & 12.80 [10.21–15.39] & 15.15 [13.79–16.51] & 14.17 [10.11–18.22]
& – & – & – \\
& & Gap    & – & – & – & 1.30 [-0.14–2.74] & 0.68 [-0.10–1.46] & 0.70 [-0.29–1.65] \\
\midrule

\multirow{4}{*}{Dalia} & \multirow{4}{*}{MIMIC}
& Total  & 22.72 [21.54–23.91] & 22.46 [21.05–23.86] & 22.70 [20.05–25.35]
& – & – & – \\
& & Male   & 22.07 [20.78–23.36] & 21.71 [20.20–23.22] & 21.98 [19.06–24.89]
& – & – & – \\
& & Female & 23.13 [22.00–24.26] & 22.91 [21.62–24.20] & 23.13 [20.63–25.64]
& – & – & – \\
& & Gap    & – & – & – & 1.06 [0.91–1.21] & 1.20 [0.90–1.50] & 1.16 [0.71–1.60] \\
\midrule


\bottomrule
\end{tabular}
\label{tab:mae_fairness}
\end{table*}
